DRSM: De-Randomized Smoothing on Malware Classifier Providing Certified Robustness

Machine Learning (ML) models have been utilized for malware detection for over two decades. Consequently, this ignited an ongoing arms race between malware authors and antivirus systems, compelling researchers to propose defenses for malware-detection models against evasion attacks. However, most if not all existing defenses against evasion attacks suffer from sizable performance degradation and/or can defend against only specific attacks, which makes them less practical in real-world settings. In this work, we develop a certified defense, DRSM (De-Randomized Smoothed MalConv), by redesigning the de-randomized smoothing technique for the domain of malware detection. Specifically, we propose a window ablation scheme to provably limit the impact of adversarial bytes while maximally preserving local structures of the executables. After showing how DRSM is theoretically robust against attacks with contiguous adversarial bytes, we verify its performance and certified robustness experimentally, where we observe only marginal accuracy drops as the cost of robustness. To our knowledge, we are the first to offer certified robustness in the realm of static detection of malware executables. More surprisingly, through evaluating DRSM against 9 empirical attacks of different types, we observe that the proposed defense is empirically robust to some extent against a diverse set of attacks, some of which even fall out of the scope of its original threat model. In addition, we collected 15.5K recent benign raw executables from diverse sources, which will be made public as a dataset called PACE (Publicly Accessible Collection(s) of Executables) to alleviate the scarcity of publicly available benign datasets for studying malware detection and provide future research with more representative data of the time.

==> sections/discussion.tex <==
\label{ref:discussion}

==> sections/prev_abstract.tex <==
%Machine Learning (ML) models have been utilized for malware detection for over two decades. Consequently, this gave rise to an ongoing arms race between malware authors and antivirus systems, and researchers have proposed mechanisms for defending malware-detection models against evasion attacks. However, the existing defenses against evasion attacks suffer from performance degradation and/or can defend against only specific attacks, which make them less practical in real-life settings. We study this trade-off under multiple adversarial settings and present DRSM (De-Randomized Smoothed MalConv) as a certified defense, which combines our adapted *de-randomized smoothing* technique with state-of-the-art CNN-based malware classifiers. Benefit from the *window ablation smoothing* scheme we propose, the impact of adversarial perturbation is mitigated while the malicious features of a malware file can still be learned. We analyze how different ablation parameters in DRSM can impact standard and certified accuracy, and compare it to the base classifier. To our knowledge, we are the first to introduce certified robustness in the realm of malware detection. Beyond our theoretical formulations, we extensively evaluate our DRSM model against $9$ different attacks in both white-box and black-box settings. Notably, we deliberately include some practical attacks that fall outside of our threat model to showcase the applicability of our proposed method. We then discuss some insights gained from our results. Moreover, due to the scarcity of publicly available benign datasets in the malware domain, we collected $15.5K$ very recent benign raw executables from different sources throughout this work. We are going to publish the dataset following the common standard and guidelines, to allow future research to curate a diverse set of benign programs for experiments that are more representative of the real-world. To facilitate the reproducibility of our findings, we build our framework on top of 'secml-malware' Python library, and open-source the implementation.
